GECTurk WEB: An Explainable Online Platform for Turkish Grammatical Error Detection and Correction

Sophisticated grammatical error detection/correction tools are available for a small set of languages such as English and Chinese. However, it is not straightforward -- if not impossible -- to adapt them to morphologically rich languages with complex writing rules like Turkish which has more than 80 million speakers. Even though several tools exist for Turkish, they primarily focus on spelling errors rather than grammatical errors and lack features such as web interfaces, error explanations and feedback mechanisms. To fill this gap, we introduce GECTurk WEB, a light, open-source, and flexible web-based system that can detect and correct the most common forms of Turkish writing errors, such as the misuse of diacritics, compound and foreign words, pronouns, light verbs along with spelling mistakes. Our system provides native speakers and second language learners an easily accessible tool to detect/correct such mistakes and also to learn from their mistakes by showing the explanation for the violated rule(s). The proposed system achieves 88,3 system usability score, and is shown to help learn/remember a grammatical rule (confirmed by 80% of the participants). The GECTurk WEB is available both as an offline tool at https://github.com/GGLAB-KU/gecturkweb or online at www.gecturk.net.

==> table.tex <==
    \begin{table*}
        \centering
        \scalebox{0.8}{
            \begin{tabular}{
              >{\centering\arraybackslash}m{2cm}
              >{\centering\arraybackslash}m{4cm}
              >{\centering\arraybackslash}m{2cm}
              >{\centering\arraybackslash}m{2cm}
              >{\centering\arraybackslash}m{3cm}
            }
            \toprule
             \textbf{No} & \textbf{Question} & \textbf{Mean} & \textbf{Range} & \textbf{Better}\\
            \toprule
            1 & I think that I would like to use this system frequently. & 4.5 & [1, 5] & $\uparrow$ \\
            \midrule
            2 & I found the system unnecessarily complex. & 1.0 & [1, 5] & $\downarrow$ \\ 
            \midrule
            3 & I thought the system was easy to use. & 5.0 & [1, 5] & $\uparrow$ \\ 
            \midrule        
            4 & I think that I would need the support of a technical person to be able to use this system. & 1.0 & [1, 5] & $\downarrow$ \\ 
            \midrule
            5 & I found the various functions in this system were well integrated. & 4.4 & [1, 5] & $\uparrow$ \\ 
            \midrule
            6 & I thought there was too much inconsistency in this system. & 1.5 & [1, 5] & $\downarrow$ \\ 
            \midrule        
            7 & I would imagine that most people would learn to use this system very quickly. & 5.0 & [1, 5] & $\uparrow$ \\ 
            \midrule        
            8 & I found the system very cumbersome to use. & 1.2 & [1, 5] & $\downarrow$ \\ 
            \midrule        
            9 & I felt very confident using the system. & 4.8 & [1, 5] & $\uparrow$ \\ 
            \midrule        
            10 & I needed to learn a lot of things before I could get going with this system. & 1.0 & [1, 5] & $\downarrow$ \\        
            \midrule
            11 & The website is easy to use. & 5.0 & [1, 5] & $\uparrow$ \\ 
            \midrule
            12 & It is easy to navigate within the website. & 5.0 & [1, 5] & $\uparrow$ \\ 
            \midrule
            13 & The information on the website is credible. & 4.3 & [1, 5] & $\uparrow$ \\ 
            \midrule
            14 & The information on the website is trustworthy. & 4.0 & [1, 5] & $\uparrow$ \\ 
            \midrule
            15 & I find the website to be attractive. & 4.4 & [1, 5] & $\uparrow$ \\ 
            \midrule
            16 & The website has a clean and simple presentation. & 4.8 & [1, 5] & $\uparrow$ \\ 
            \midrule
            17 & I will likely return to the website in the future. & 4.2 & [1, 5] & $\uparrow$ \\ 
            \midrule
            18 & How likely are you to recommend the website to a friend or colleague? & 8.3 & [0, 10] & $\uparrow$ \\ 
            \midrule
            19 & I learned a new rule and/or remembered a rule I had forgotten. & 0.8 & 0 or 1 & $\uparrow$ \\ 
            \bottomrule
            \end{tabular}   
        }
    \caption{The list of questions for the second part of the user study. \textbf{No:} There are total 19 questions, 1-10 are from SUS, 11-18 are from SUPR-Q, and the last question is to measure tool's impact on learning and retention. \textbf{Better:} Indicates which score is better: Higher ($\uparrow$) or Lower. ($\downarrow$)}
    \label{table:4}
    \end{table*}
